Preference Conditioned Multi-Objective Reinforcement Learning: Decomposed, Diversity-Driven Policy Optimization

Multi-objective reinforcement learning (MORL) seeks to train agents capable of balancing conflicting objectives. While single preference-conditioned policies offer a highly scalable solution, existing approaches remain brittle in practice, frequently failing to recover dense Pareto fronts. We demonstrate that this failure stems from two structural pathologies: destructive advantage cancellation caused by premature Early Scalarization (ES), and representational mode collapse across the preference space. To overcome these bottlenecks, we introduce $D^3PO$, a PPO-based framework that fundamentally reorganizes multi-objective optimization. By preserving per-objective learning signals through a decomposed pipeline and integrating preferences only after trust-region stabilization (Late-Stage Weighting), $D^3PO$ improves credit assignment under conflicting objectives. Concurrently, a scaled diversity regularizer encourages behavioral divergence proportional to preference distance. $D^3PO$ operates entirely within the efficient linear scalarization regime shared by standard deep MORL baselines. By reducing information loss caused due to linear scalarization rather than relying on expensive non-linear utility functions, it suggests that optimization bottlenecks play a significant role. Across available standard benchmarks, including high-dimensional and many-objective environments, $D^3PO$ consistently discovers broader, higher-quality Pareto fronts than prior methods, exceeding state-of-the-art hypervolume and expected utility using a single deployable policy.

==> 0-TODO_LIST.tex <==
Rebuttal document is here:

\url{https://docs.google.com/document/d/1dnumpDhpUkzmK8nb1dtGmJ1jYxYJT55QXSrv_xMnSJ8/edit?tab=t.0}

==> 00-titleAuthorAbstract.tex <==
\title{%Why Constrain Ourselves? Multi-Objective Reinforcement Learning with Non-Convex Weighting \\
%Learning a Single, Generalizable Policy for Multi-Objective Reinforcement Learning\\
%A Decomposed, Diversity-Driven Framework for Multi-Objective Reinforcement Learning\\
% Learning a Single Generalizable Policy for Multi Objective Reinforcement Learning with Decomposed, Diversity-Driven PPO
% \\
% Learning a Single Generalizable Policy for Multi Objective RL with Decomposed, Diversity-Driven PPO
% \\
Preference Conditioned Multi-Objective Reinforcement Learning: Decomposed, Diversity-Driven Policy Optimization
% \\\\
% Learning Single Generalizable Multi-Objective Reinforcement Learning Policies
% Learning a <PROPERTIES> Policy for MORL with <ALG>

% Title idea 3}
}
%JED: go ahead and put any title brainstorms you have here, formatted as illustrated. Once we have a few on the rack, we can discuss as a group what we like about each one and hybridize them into the final copy

%JED: I'll suggest the author order for this one be: Tanmay, Sourav, Shreyash, any kitware folks, Me, Abhinav
%JED: I texted Brian, we cannot do a public release request in time, so the kitware folks must remain in acknowledgment for this one, if accepted. We can rethink if rejected


% The \author macro works with any number of authors. There are two commands
% used to separate the names and addresses of multiple authors: \And and \AND.
%
% Using \And between authors leaves it to LaTeX to determine where to break the
% lines. Using \AND forces a line break at that point. So, if LaTeX puts 3 of 4
% authors names on the first line, and the last on the second line, try using
% \AND instead of \And before the third author name.


\author{%
  David S.~Hippocampus\thanks{Use footnote for providing further information
    about author (webpage, alternative address)---\emph{not} for acknowledging
    funding agencies.} \\
  Department of Computer Science\\
  Cranberry-Lemon University\\
  Pittsburgh, PA 15213 \\
  \texttt{hippo@cs.cranberry-lemon.edu} \\
  % examples of more authors
  % \And
  % Coauthor \\
  % Affiliation \\
  % Address \\
  % \texttt{email} \\
  % \AND
  % Coauthor \\
  % Affiliation \\
  % Address \\
  % \texttt{email} \\
  % \And
  % Coauthor \\
  % Affiliation \\
  % Address \\
  % \texttt{email} \\
  % \And
  % Coauthor \\
  % Affiliation \\
  % Address \\
  % \texttt{email} \\
}

\newcommand{\abstractText}[1]{%
%``Dr. Burnett's Formula'': 
% 1. What's the problem
% 2. Why is the problem a problem
% 3. What did we do about it?
% 4. What did that do for the world OR what are 1-2 interesting things we found out?

Multi-objective reinforcement learning (MORL) aims to optimize policies in environments with multiple, often conflicting objectives. While a single, preference-conditioned policy offers the most flexible and efficient solution, existing methods often struggle to cover the entire spectrum of optimal trade-offs. This is frequently due to two underlying challenges: destructive gradient interference between conflicting objectives and representational mode collapse, where the policy fails to produce diverse behaviors. In this work, we introduce \toolname{}, a novel algorithm that trains a single preference conditioned policy to directly address these issues. Our framework features a decomposed optimization process to encourage stable credit assignment and a scaled diversity regularizer to explicitly encourage a robust mapping from preferences to policies. Empirical evaluations across six standard MORL benchmarks show that \toolname{} discovers more comprehensive and higher-quality Pareto fronts, establishing a new state-of-the-art in terms of hypervolume and expected utility, particularly in complex and many-objective environments.

}


==> documentBody/H-convergence.tex <==
\section{Theoretical Analysis of Convergence}
\label{sec:convergence}

We analyze the convergence behavior of preference-conditioned actor updates with the scaled diversity regularizer. We first consider an idealized tabular setting, where convergence to stationary points can be established under exact gradients. We then extend the analysis to the function-approximation regime, where stochastic approximation theory provides guarantees under standard smoothness and noise assumptions.

\begin{theorem}[Convergence to Stationary Points in the Tabular Setting]
\label{thm:tabular_convergence}
Assume:
\begin{enumerate}
    \item The environment is a finite MDP with bounded rewards and finite state and action spaces.
    \item The policy is parameterized in tabular form, i.e., each state--preference pair $(s,\omega)$ has an independent probability distribution over actions.
    \item The exact expected actor objective $J(\pi)$, including the scaled diversity regularizer, is available, and exact gradients with respect to $\pi$ can be computed.
    \item $J(\pi)$ is continuously differentiable with Lipschitz continuous gradients.
    \item Gradient ascent is performed with a sufficiently small constant step size or a diminishing step-size schedule.
\end{enumerate}
Then gradient ascent converges to the set of stationary points of $J(\pi)$.
\end{theorem}

\begin{proof}[Proof sketch]
In the tabular parameterization, the optimization variables are the policy probability vectors 
$\{\pi(\cdot|s,\omega)\}$, one for each state--preference pair $(s,\omega)$. These variables lie in a product of probability simplices, which is compact.

The policy improvement term of the actor objective is a smooth function of $\pi$. The scaled diversity regularizer involves squared deviations of KL divergences, which are generally nonconvex functions of $\pi$. As a result, the combined actor objective $J(\pi)$ is continuously differentiable but not necessarily concave.

Under the stated smoothness assumptions and compactness of the domain, standard results on gradient ascent for smooth nonconvex objectives imply convergence to the set of stationary points of $J(\pi)$.

Thus, while global optimality cannot be guaranteed due to nonconvexity, convergence to stationary points holds in the tabular setting.
\end{proof}


\begin{theorem}[Convergence to Stationary Points with Function Approximation]
\label{thm:stationary_convergence}
Let $J(\theta)$ denote the expected actor objective, including the scaled diversity regularizer, and assume:
\begin{enumerate}
    \item $J(\theta)$ is continuously differentiable and $L$-smooth.
    \item The stochastic gradient estimators $\hat g_t$ approximate $\nabla J(\theta_t)$ with bounded variance:
    \[
        \mathbb{E}\|\hat g_t - \nabla J(\theta_t)\|^2 \leq \sigma^2.
    \]
    \item The step-sizes $\{\eta_t\}$ satisfy the Robbins--Monro conditions:
    \[
        \sum_{t=1}^{\infty} \eta_t = \infty, 
        \quad \sum_{t=1}^{\infty} \eta_t^2 < \infty.
    \]
    \item The parameter sequence $\{\theta_t\}$ remains in a compact set or is projected onto one.
\end{enumerate}
Then
\[
    \lim_{t \to \infty} \|\nabla J(\theta_t)\| = 0
\quad \text{almost surely under these assumptions}.
\]
\end{theorem}

\begin{proof}[Proof sketch]
The actor parameters are updated according to
\[
    \theta_{t+1} = \theta_t + \eta_t \hat g_t.
\]

Under $L$-smoothness of $J$, the associated mean ODE
\[
    \dot{\theta} = \nabla J(\theta)
\]
has Lipschitz continuous dynamics. The bounded-variance assumption ensures that stochastic perturbations do not dominate the updates, while the Robbins--Monro step-size conditions guarantee diminishing noise influence. Compactness of the parameter domain ensures bounded iterates.

Standard stochastic approximation results imply that the iterates $\{\theta_t\}$ track the mean ODE asymptotically, and their limit set is contained within the set of stationary points of $J$. Consequently,
\[
    \lim_{t \to \infty} \|\nabla J(\theta_t)\| = 0
\]
under the stated assumptions.
\end{proof}

\paragraph{Interpretation.}
The tabular result establishes convergence to stationary points under exact gradients, reflecting the nonconvexity introduced by the scaled diversity regularizer. In the function-approximation regime, convergence to stationary points follows from standard stochastic approximation theory under smoothness and bounded-noise assumptions.

These guarantees are comparable to those typically available for modern policy gradient methods. As in those settings, the results rely on standard assumptions that abstract away distributional shift and approximation error inherent in reinforcement learning. Within this framework, the analysis provides a theoretical basis for the stability observed empirically.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> table/OLD-compute_time.tex <==
\begin{table*}[!htb]
\centering
\begin{tabular}{llllll}
\toprule
\textbf{Environments (Hypervolume $\uparrow$)} & \textbf{CAPQL} & \textbf{PG-MORL} & \textbf{GPI-LS} & \textbf{C-MORL} & \textbf{\toolname{}} \\ \midrule

MO-Hopper-2d ($10^5$) & $1.15 \pm 0.08$ & $1.20 \pm 0.09$ & $1.19 \pm 0.10$ & $\mathbf{1.37 \pm 0.03}$ & $1.30 \pm 0.03$ \\
\midrule
MO-Hopper-3d ($10^7$) & $1.65 \pm 0.45$ & $1.59 \pm 0.45$ & $1.70 \pm 0.29$ & $\mathbf{2.19 \pm 0.32}$ & $2.12\pm 0.16$ \\ \midrule
MO-Ant-2d ($10^5$) & $1.11 \pm 0.69$ & $0.35 \pm 0.08$ & $1.17 \pm 0.25$ & $1.31 \pm 0.16$ & $\mathbf{1.91 \pm 0.18}$ \\ \midrule
MO-Ant-3d ($10^7$) & $1.22 \pm 0.33$ & $0.94 \pm 0.12$ & $0.55 \pm 0.81$ & $2.61 \pm 0.26$ & $\mathbf{2.68 \pm 0.21}$ \\ \midrule
MO-Humanoid-2d ($10^5$) & $3.30 \pm 0.06$ & $2.62 \pm 0.32$ & $1.98 \pm 0.02$ & $3.43 \pm 0.06$ & $\mathbf{3.76 \pm 0.11}$ \\ \midrule
Building-9d ($10^{31}$) & $4.29 \pm 0.73$ & T/O & T/O & $7.93 \pm 0.07$ & $\mathbf{8.00 \pm 0.11}$ \\

\bottomrule
\end{tabular}
\caption{Performance comparison across continuous environments based on the Hypervolume (HV) metric. Higher is better.}
\label{tab:compute-results}
\end{table*}

==> table/OLD-continuous.tex <==
\begin{table*}[!htb]
\centering
\begin{tabular}{lllllll}
\toprule
\textbf{Environments} & \textbf{Metrics} & \textbf{CAPQL} & \textbf{PG-MORL} & \textbf{GPI-LS} & \textbf{C-MORL} & \textbf{\toolname{}} \\ \midrule

\multirow{3}{*}{MO-Hopper-2d} 
& HV ($10^5 \uparrow$)     & $1.15 \pm 0.08$ & $1.20 \pm 0.09$ & $1.19 \pm 0.10$ & $\mathbf{1.37 \pm 0.03}$ & $1.30 \pm 0.03$ \\
& EU ($10^2 \uparrow$)     & $2.28 \pm 0.07$ & $2.34 \pm 0.10$ & $2.33 \pm 0.10$ & $\mathbf{2.53 \pm 0.02}$ & $2.47 \pm 0.01$ \\
& SP ($10^2 \downarrow$)     & $0.46 \pm 0.10$ & $5.13 \pm 5.81$ & $0.49 \pm 0.37$ & $1.13 \pm 0.19$ & $\mathbf{0.26 \pm 0.31}$ \\ \hline

\multirow{3}{*}{MO-Hopper-3d} 
& HV ($10^7 \uparrow$)     & $1.65 \pm 0.45$ & $1.59 \pm 0.45$ & $1.70 \pm 0.29$ & $\mathbf{2.19 \pm 0.32}$ & $2.12\pm 0.16$ 
\\
& EU ($10^2 \uparrow$)     & $1.53 \pm 0.28$ & $1.47 \pm 0.25$ & $1.62 \pm 0.10$ & $\mathbf{1.81 \pm 0.01}$ & $1.74 \pm 4.9$ \\
& SP ($10^2 \downarrow$)     & $2.31 \pm 3.16$ & $0.76 \pm 0.91$ & $0.74 \pm 1.22$ & $0.53 \pm 0.34$ & $\mathbf{0.04 \pm 0.01}$ \\ \hline

\multirow{3}{*}{MO-Ant-2d} 
& HV ($10^5 \uparrow$)     & $1.11 \pm 0.69$ & $0.35 \pm 0.08$ & $1.17 \pm 0.25$ & $1.31 \pm 0.16$ & $\mathbf{1.91 \pm 0.18}$ \\
& EU ($10^2 \uparrow$)     & $2.16 \pm 0.94$ & $0.81 \pm 0.23$ & $4.28 \pm 0.19$ & $2.50 \pm 0.25$ & $\mathbf{3.14 \pm 0.21}$ \\
& SP ($10^3 \downarrow$)     & $\mathbf{0.18 \pm 0.07}$ & $2.20 \pm 3.48$ & $3.61 \pm 2.13$ & $2.65 \pm 1.25$ & $0.66 \pm 0.40$ \\ \hline

\multirow{3}{*}{MO-Ant-3d} 
& HV ($10^7 \uparrow$)     & $1.22 \pm 0.33$ & $0.94 \pm 0.12$ & $0.55 \pm 0.81$ & $2.61 \pm 0.26$ & $\mathbf{2.68 \pm 0.21}$ \\
& EU ($10^2 \uparrow$)     & $1.30 \pm 0.29$ & $1.07 \pm 0.07$ & $2.41 \pm 0.20$ & $\mathbf{2.06 \pm 0.14}$ & $1.99 \pm 0.08$ \\
& SP ($10^3 \downarrow$)     & $0.17 \pm 0.09$ & $0.02 \pm 0.01$ & $1.96 \pm 0.79$ & $0.06 \pm 0.07$ & $\mathbf{0.004 \pm 0.002}$ \\ \hline

\multirow{3}{*}{MO-Humanoid-2d} 
& HV ($10^5 \uparrow$)     & $3.30 \pm 0.06$ & $2.62 \pm 0.32$ & $1.98 \pm 0.02$ & $3.43 \pm 0.06$ & $\mathbf{3.76 \pm 0.11}$ \\
& EU ($10^2 \uparrow$)     & $4.75 \pm 0.04$ & $4.06 \pm 0.32$ & $3.67 \pm 0.02$ & $4.78 \pm 0.05$ & $\mathbf{5.11 \pm 0.09}$ \\
& SP ($10^4 \downarrow$)     & $\mathbf{0.00 \pm 0.00^*}$ & $0.13 \pm 0.17$ & $\mathbf{0.00 \pm 0.00^*}$ & $2.21 \pm 3.47$ & $\mathbf{0.003 \pm 0.001}$ \\ \hline

\multirow{3}{*}{Building-9d} 
& HV ($10^{31} \uparrow$)     & $4.29 \pm 0.73$ & T/O & T/O & $7.93 \pm 0.07$ & $\mathbf{8.00 \pm 0.11}$ \\
& EU ($10^3 \uparrow$)        & $3.31 \pm 0.06$ & T/O & T/O & $3.50 \pm 0.00$ & $\mathbf{3.50 \pm 0.003}$ \\
& SP ($10^3 \downarrow$)        & $4.34 \pm 3.72$ & T/O & T/O & $2.79 \pm 0.40$ & $\mathbf{0.03 \pm 0.01}$ \\

\bottomrule
\end{tabular}
\caption{Performance comparison across continuous environments.
learning only one point is considered good
}
\label{tab:continous-results}
\end{table*}



==> table/OLD-mine+lunar.tex <==
\begin{table*}[!htb]
\centering
\begin{tabular}{llllll}
\toprule
\textbf{Environments} & \textbf{Metrics} & \textbf{GPI-LS} & \textbf{C-MORL} & \textbf{\toolname{}} \\ \midrule
\multirow{4}{*}{\textbf{Minecart}} 
& HV ($10^2 \uparrow$)     &$6.05 \pm 0.37$ & $7.72  \pm 0.7$ & $\mathbf{6.56 \pm 0.42}$ \\ 
& EU ($10^{-1} \uparrow$)  &$2.29 \pm 0.32 $ & $\mathbf{2.65 \pm 0.37}$ & $1.4 \pm 0.1$ \\
& SP ($10^{-1} \downarrow$)  & $0.10 \pm 0.00$ & $0.09 \pm 0.03$ & $\mathbf{0.01 \pm 0.01}$ \\
\hline
\multirow{4}{*}{\textbf{Lunar Lander-4d}} 
& HV ($10^9 \uparrow$)     &$1.06 \pm 0.16$ & $\mathbf{1.12 \pm 0.03}$ & $\mathbf{1.12 \pm 0.91}$ \\ 
& EU ($10^1 \uparrow$)  &$ 1.81 \pm 0.34$ & $\mathbf{2.35 \pm 0.18}$ & $2.08 \pm 0.15$ \\
& SP ($10^3 \downarrow$)  & $0.13 \pm 0.01$ & $ 1.04 \pm  0.24$ & $\mathbf{0.03 \pm 0.02}$ \\
\bottomrule
\end{tabular}
\caption{Performance comparison (Hypervolume, Expected Utility, Sparsity) on the Minecart and LunarLander environments.}
\label{tab:minecart-results}
\end{table*}
